Generalized Jensen-Shannon Divergence Loss for Learning with Noisy Labels

Prior works have found it beneficial to combine provably noise-robust loss functions e.g., mean absolute error (MAE) with standard categorical loss function e.g. cross entropy (CE) to improve their learnability. Here, we propose to use Jensen-Shannon divergence as a noise-robust loss function and show that it interestingly interpolate between CE and MAE with a controllable mixing parameter. Furthermore, we make a crucial observation that CE exhibit lower consistency around noisy data points. Based on this observation, we adopt a generalized version of the Jensen-Shannon divergence for multiple distributions to encourage consistency around data points. Using this loss function, we show state-of-the-art results on both synthetic (CIFAR), and real-world (e.g., WebVision) noise with varying noise rates.

==> Figures/app_table_hp_1.tex <==
\begin{tabular}{ @{}l l c c@{}} %@{} removes space to vertical edges
 \toprule
 \multirow{2}{4em}{Dataset} & \multirow{2}{4em}{Method} & \multicolumn{1}{c}{Sym Noise} & \multicolumn{1}{c}{Asym Noise} \\ \cmidrule(lr){3-3} \cmidrule(lr){4-4}
 & & 20-80\% & 20-40\% \\
 \midrule
 \multirow{8}{5em}{CIFAR-10} & CE & [0.05, 1e-3] & [0.1, 1e-3] \\
 & BS & [0.1, 1e-3] & [0.1, 1e-3] \\
 & LS & [0.1, 5e-4] & [0.1, 1e-3] \\
 & SCE & [0.01, 5e-4] & [0.05, 1e-3] \\
 & GCE & [0.01, 5e-4] & [0.1, 1e-3] \\
 & NCE+RCE & [0.005, 1e-3] & [0.05, 1e-4] \\
 & JS & [0.01, 5e-4] & [0.1, 1e-3] \\
 & GJS & [0.1, 5e-4] & [0.1, 1e-3] \\
\midrule
%-----------------------------------------------------
%-----------------------------------------------------
 \multirow{8}{5em}{CIFAR-100} & CE & [0.4, 1e-4] & [0.2, 1e-4] \\
 & BS & [0.4, 1e-4] & [0.4, 1e-4] \\
 & LS & [0.2, 5e-5] & [0.4, 1e-4] \\
 & SCE & [0.2, 1e-4] & [0.4, 5e-5] \\
 & GCE & [0.4, 1e-5] & [0.2, 1e-4] \\
 & NCE+RCE & [0.2, 5e-5] & [0.2, 5e-5] \\
 & JS & [0.2, 1e-4] & [0.1, 1e-4] \\
 & GJS & [0.2, 5e-5] & [0.4, 1e-4] \\
 \bottomrule
\end{tabular}


==> Figures/app_table_hp_2.tex <==
\begin{tabular}{ @{}l l c c c c c c c@{}} %@{} removes space to vertical edges
 \toprule
 \multirow{2}{4em}{Dataset} & \multirow{2}{4em}{Method} & No Noise & \multicolumn{4}{c}{Sym Noise} & \multicolumn{2}{c}{Asym Noise} \\ \cmidrule(lr){3-3}\cmidrule(lr){4-7} \cmidrule(lr){8-9}
 & & 0\% & 20\% & 40\% & 60\% & 80\% & 20\% & 40\% \\
 \midrule
 \multirow{8}{5em}{CIFAR-10} %& CE & -  & - & - & - & - & - \\
 & CE & - & - & - & - & - & - & - \\
 & BS & 0.5 & 0.5 & 0.7 & 0.7 & X & 0.7 & 0.5 \\
 & LS & 0.1 & 0.5 & 0.9 & 0.7 & X & 0.1 & 0.1 \\
 & SCE & [0.2, 0.1] & [0.05, 0.1] & [0.1, 0.1] & [0.2, 1.0] & [X,X] & [0.1, 0.1] & [0.2, 1.0] \\
& GCE & 0.5 & 0.7 & 0.7 & 0.7 & X & 0.1 & 0.1 \\
 & NCE+RCE & [10, 0.1] & [10, 0.1] & [10, 0.1] & [1.0, 0.1] & [X,X] & [10, 0.1] & [1.0, 0.1] \\
  & JS & 0.1 & 0.7 & 0.7 & 0.9 & X & 0.3 & 0.3 \\
 & GJS & 0.5 & 0.3 & 0.9 & 0.1 & X & 0.3 & 0.3 \\
\midrule
%-----------------------------------------------------
%-----------------------------------------------------
 \multirow{8}{5em}{CIFAR-100} %& CE & - & - & - & - & - & - \\
 & CE & - & - & - & - & - & - \\
 & BS & 0.7 & 0.5 & 0.5 & 0.5 & 0.3 & 0.3 \\
 & LS & 0.1 & 0.7 & 0.7 & 0.7 & 0.5 & 0.7 \\
 & SCE & [0.1, 0.1] & [0.1, 0.1] & [0.1, 0.1] & [0.1, 1.0] & [0.1, 1.0] & [0.1, 1.0] \\
 & GCE & 0.5 & 0.5 & 0.5 & 0.7 & 0.7 & 0.7 \\
 & NCE+RCE & [20, 0.1] & [20, 0.1] & [20, 0.1] & [20, 0.1] & [20, 0.1] & [10, 0.1] \\
 & JS & 0.1 & 0.1 & 0.3 & 0.5 & 0.5 & 0.5 \\
 & GJS & 0.3 & 0.3 & 0.5 & 0.9 & 0.5 & 0.1 \\
 \bottomrule
\end{tabular}
